FPR Estimation for Fraud Detection in the Presence of Class-Conditional Label Noise

We consider the problem of estimating the false-/ true-positive-rate (FPR/TPR) for a binary classification model when there are incorrect labels (label noise) in the validation set. Our motivating application is fraud prevention where accurate estimates of FPR are critical to preserving the experience for good customers, and where label noise is highly asymmetric. Existing methods seek to minimize the total error in the cleaning process - to avoid cleaning examples that are not noise, and to ensure cleaning of examples that are. This is an important measure of accuracy but insufficient to guarantee good estimates of the true FPR or TPR for a model, and we show that using the model to directly clean its own validation data leads to underestimates even if total error is low. This indicates a need for researchers to pursue methods that not only reduce total error but also seek to de-correlate cleaning error with model scores.

==> garbage.tex <==






All of our data will have timestamps associated with it, and so there is some choice in how to select training, validation, and test data as well as how to slice training data for micro-models. We will always choose the test data to follow all training and validation data in time, but otherwise will not separate training and validation data, and will shuffle training data before slicing for micro-models. This follows the approach of \cite{sabzevari2018two} and \cite{samami2020mixed}, vs. slices taken with respect to time as in \cite{cretu2008casting}. We then train a model on each slice, and then have each resulting model score every example in the held-out validation set. For each example, we record whether each model scored the example as fraudulent using a simple threshold of $0.5$, and record the fraction of models voting to classify as fraud in this way. We can determine a voting threshold so that $p(c=1) = p(y=1)$, up to some quantization. It may be interesting in future work to explore the effect of out-of-time validation and/or slicing with respect to time but we do not discuss it further here.

Once the validation data has been cleaned, we will train a model on the entire set of training data, validate it on the cleaned data (choose a threshold that achieves our target FPR on the validation data), and then score a set of held-out test data. This test data is labelled and we assume the labels are clean. We measure the FPR on this test data and hope that we improve the FPR targeting. One fact which is obvious with thought but bears mention is that \textit{underestimating} FPR in validation will lead to \textit{overshooting} FPR in test, and vice-versa. 
























unused:
On the other hand, consider some method $c$ so that there is some example $(x,y^*=0,y=0)$ with $f(x) < \tau$ but $c(x,y^*) = 1$, i.e. this is a low-scoring type-1 error for $c$. Note that by symmetry there must also be a high-scoring type-2 error for this method, $(x,y^*=0,y=1)$ with $f(x)>\tau$ but $c(x,y^*) = 0$. The first observation implies 
    \begin{align}
    
        p(f > t | y = 0, c=1) < 1 = p(f > t | y = 0, \wt{c}=1).
    \end{align}



the study of the effect of noise in the validation (vs. training) process as well as the study of how different approaches to slicing the training data yield more or less effective cleaning ensembles. We also derive an identity relating the error in the FPR estimate to the correlation between the error in the cleaning process and the ``base model'' score used to set an FPR threshold which motivates the use of ensemble methods over the ``base model'' score (as in CleanLab).


; we will first do this under the assumption that the noise level is known (but the specific examples are not), and then we will attempt to remove noise without this assumption. We will  In each case, we will measure success in terms of the error in the estimate of FPR obtained on noisy validation data vs. the actual FPR on a clean test set.

 

call to action





Further it is also typical to assume that noise is independent of the features, in other words that the probability of observing a label $y^*$ depends only on the true label $y$ and not the features $x$. This assumption is unrealistic in our applications where adversarial behavior is exhibited (bad actors change their behavior over time to evade detection) or where some time may elapse between account creation, credit application, etc. and the eventual fraud decision - that is, the labels are initially noisy and then later corrected. In practical application we would typically like to use the most recent data to the greatest extent possible in order to capture the most recent trends, but this issue of label maturity makes this difficult - in our experiments (see Table \ref{tab:exact_cloud}) we see that FPR is underestimate by as much as $80\%$ if no cleaning is done; cleaning label noise provides a way to leverage recent data and still obtain accurate FPR estimates.

this work we will not attempt to explicitly diagnose the cause of label noise, and will find it sufficient to build our intuition around label maturity. 

 This will indicate a need for investigate the theoretical basis for our technique providing a good estimate of the FPR. As noted earlier, we will find it useful to have micro-models that give predictions that are somewhat independent of each other, and independent of scores from our final classifier.
 
 
  - if we knew enough about the actual labels, then we could experimentally determine an optimal threshold but this may not be reasonable in practice (if we always had such information there would be no need to use such a technique to remove noise!). Thus we must either make a consistent choice (e.g. to always use majority voting) and verify its results in a variety of settings, or come up with ways to find an optimal threshold that do not depend on knowledge of the true labels.
  
  
  
  
  ***old final sections***
  
  \subsection{Our approach}

In our situation we will take a simple approach and just use majority voting. Our approach also differs from \cite{samami2020mixed} in that they use five different types of classifiers and a leave-one-out approach to the folds, where we use the same type of classifier throughout the ensemble and train each model on only one fold. Thus we expect each model to be relatively weak, but relatively independent which we will find desirable.  

Additional novelty here is careful attention to what data is used to train the micro-models and then observation of how this effects FPR targeting rather than accuracy. In particular, given a dataset that includes labels and timestamps, we will first split the data into training and validation sets, possibly using the timestamp to split (but not otherwise using the timestamp as a feature). We will then split the training data into smaller slices, using the timestamps to do this (following \cite{cretu2008casting}) or randomly (as in most other approaches including \cite{sabzevari2018two} and \cite{samami2020mixed}). We then train a model on each slice, and then have each resulting model score every example in the held-out validation set. For each example, we record whether each model scored the example as fraudulent using a simple threshold of $0.5$, and then mark any example with $y^*=0$ as noise if a majority of the ensemble voted to classify it as fraud.

We consider the following choices which need to be made in this process:
\begin{itemize}
	\item Whether to split training/validation sets in time (e.g. all training data comes before all validation data) or whether to do the assignment randomly.
	\item When splitting the training data, whether to use contiguous-in-time slices or to do the assignment randomly.
	\item How many slices to take (how many models in the ensemble). 
\end{itemize} 
We could also choose a different voting threshold other than majority (i.e. one-half of the ensemble) such as consensus, the fraud rate in training, etc. but we will not explore this here as it can be hard to validate such a choice.

Once the validation data has been cleaned, we will train a model on the entire set of training data, validate it on the cleaned data (choose a threshold that achieves our target FPR on the validation data), and then score a set of held-out test data. This test data is labelled and we assume the labels are clean. We measure the FPR on this test data and hope that we improve the FPR targeting. 



\subsection{Datasets}

To conduct our experiments we will work with some of our production data - which we will denote as the \texttt{cloud} dataset - as well as several publicly available fraud-related datasets. We cannot publish our production datasets for various reasons including protecting customer privacy, and will need to be intentionally vague about some characteristics here, but results are also demonstrated on the public datasets and can be reproduced. In the case of our production data, examples of registration data are a representative corpus of data from customers that provided permission, and were sampled from a fixed time-period ending January 1 of a recent calendar year. Any account marked fraudulent before Jan. 1 is given an accurate label of $1$ in the data, any account marked fraudulent afterward is given the noisy label of $0$. Thus this simulates the problem of training a model on extremely recent data where label maturity may be an issue. For test data, we sample examples created after Jan. 1 and assign the (to the best of our knowledge) correct labels. The features are a mixture of categorical and numeric features; examples include the country associated with the IP address used during account creation, and the number of other accounts created with the same IP address. The fraud rate in this dataset is comparable to industrial trends (between $5$ and $25\%$) and the noise rate obtained by the process above is likewise in this range.

For the public datasets, we start with the datasets made available in \cite{grover2022fdb} and choose scenarios where there is some sort of timestamp associated with the event in question. We simulate noise by adding noise weighted by the event timestamp to the training and validation data: we convert these timestamps into milliseconds elapsed since the oldest example, and then use this to weight the sampling. Overall we flip $30\%$ of the fraudulent labels to be $0$ in the training and validation data, and leave the test data clean (i.e. as-is). We then train our ensemble, clean the validation data, train/validate our final model, and evaluate on the test data.

The benchmark datasets we use are:
\begin{itemize}
	\item \texttt{ieeecis} - prepared by IEEE Computational Intelligence society, this is a set of card-not-present transactions used for a Kaggle competition. The fraud rate in this dataset is $3.5\%$ and there are 67 features, 6 of which are categorical the rest numerical.
	\item \texttt{ccfraud} - this dataset is anonymized credit card transactions from European cardholders. The fraud rate in this dataset is very low - $0.18\%$ - and all of features are numerical (obtained by using PCA on the original set of features).
	\item \texttt{fraudecom} - This is a dataset of e-commerce transactions. The fraud rate in this dataset is $10.6\%$ with 6 features: 2 categorical, 3 numeric, and IP address which we do not use. 
	\item \texttt{sparknov} - This is a simulated credit card transaction dataset generate by the Sparkov Data Generation tool. The fraud rate is $5.7\%$ and there are 17 features: 10 categorical, 6 numeric, and 1 text feature that we do not use.
\end{itemize}

We reject some of these datasets as inappropriate for this study, see Appendix \ref{fdb-no-use} for explanation.

\section{Experiment Setup}

We will conduct two types of experiments, where the noise level is known, and then where it is unknown. Throughout our key goal will be to clean noisy validation data in order to accurately target a specified FPR on clean test data.

In all cases, we will use \texttt{CatBoostClassifier}s, setting number of iterations to 100 and passing in categorical features, but otherwise doing no optimization or tuning. In both cases we will train a classifier on the entire training data and then designate this ``base model'' and set it aside. For micro-models we will train an ensemble of classifiers on sliced training data, and use them to clean the validation data. For CleanLab we will use the base model and the \texttt{find\_noisy\_labels} method to clean the data. We will then validate the base model with each validation set in this collection, taking note of the threshold determined in the validation process. Finally for each cleaning method we evaluate the base model at each corresponding threshold against clean test data and note the FPR as well as the relative error vs. the target FPR (i.e. $err = (FPR_{actual} - FPR_{target})/FPR_{target}$).

For the first set of experiments, where noise level is known, we will remove the most suspicious examples first and then proceed until we have removed the known amount of noise or until the algorithm has no more suspicious examples to consider. In the case of micro-models, we use the proportion of model votes to rank examples, stopping if no model votes to remove (i.e. there is consensus that an example is not fraudulent). For CleanLab, we use the \texttt{return\_indices\_ranked\_by=self\_confidence} parameter in order to get a ranked list of potential noise, stopping when this list runs out of candidates. Because this approach often runs out of candidates before we have reached the known noise level, we also compare a third approach where we simply rank by model score and remove the highest-scoring examples to achieve the target level of noise removal.

In the second set of experiments we make no assumption about the noise level, and use majority voting for micro-models, and the \texttt{find\_label\_issues} method in CleanLab to identify which examples to remove. After removal we validate to our target FPR and then evaluate on clean test data. 

In both cases we will consider a range of FPRs that may be realistic targets in a production setting, and determine which methods yield a test FPR closest to our target (in practice we may want to penalize more for overshooting the FPR vs. undershooting but for now we just consider the absolute magnitude of error). The FPRs we use are $0.5\%, 1\%, 2\%, 4\%, 8\%$ and $10\%$.

For training micro-models we also have a choice in how to assign training data to each model, we can either partition the data according to the timestamp or just partition randomly and we will study the effects of this choice.

We summarize these choices as follows:
\begin{itemize}
	\item Training and validation data are intermingled in time
	\begin{itemize}
		\item No cleaning is done to validation data (\textbf{[None]})
		\item CleanLab is used to clean validation data (\textbf{[CleanLab]})
		\item The base model score is used to clean validation data (\textbf{[BaseScore]})
		\item Micro-models are trained on contiguous time slices and then used to clean validation data (\textbf{[Sorted]})
		\item Micro-models are trained on random (but disjoint) subsets of the training data and then used to clean validation data (\textbf{[Shuffled]})
	\end{itemize}
	\item Training and validation data are separated in time (with training first)
	\begin{itemize}
		\item CleanLab is used to clean validation data (\textbf{[CleanLab OOT]})
		\item Micro-models are trained on contiguous time slices and then used to clean validation data (\textbf{[Sorted OOT]})
		\item Micro-models are trained on random (but disjoint) subsets of the training data and then used to clean validation data (\textbf{[Shuffled OOT]})
	\end{itemize}
\end{itemize}

Note that \textbf{BaseScore} is similar to \textbf{CleanLab} in that they both remove the highest scoring examples. They differ in that \textbf{CleanLab} will have some threshold where it stops no matter what, but \textbf{BaseScore} keeps going until we have reached our target percentage for removal. 

\section{Experiment Results}\label{results_section}

\subsection{Known Noise Level}

Generally we see micro-models perform as well or better than CleanLab in this set of experiments, though there are some cases where CleanLab performs slightly better. Both perform substantially better than the BaseScore method. Choosing an OOT training/validation split is usually preferable. In the following tables the best result at each FPR is bolded. We show full results for the \texttt{cloud} dataset in this section, and include results for the other datasets in Appendix \ref{results}.

On the \texttt{cloud} dataset (Table \ref{tab:exact_cloud}) CleanLab does slightly better than the best micro-model at the lowest FPR but is overtaken through the middle FPR ranges by the OOT micro-model methods. At the higher FPRs ($8\%$ and $10\%$) all micro-model methods perform significantly better than CleanLab. As expected, the BaseScore method is very error-prone especially at the lowest FPR targets, though at high FPR targets this aggressive approach produces acceptable results and CleanLab is probably not aggressive enough (though this is still not enough to recommend BaseScore in the general setting).

On the \texttt{ieeecis} dataset (Table \ref{tab:exact_ieeecis}) CleanLab methods outperform all other methods across the range of FPRs, though the advantage diminishes at the higher targets. Again, the BaseScore method exhibits drastic overshoot at low FPRs and is uniformly the worst method.

On the \texttt{ccfraud} dataset (Table \ref{tab:exact_ccfraud}) all methods perform comparably. This is possibly due to the fact that classes are very imbalanced in this data and so adding or cleaning noise does not do much to the calculation of the false positive rate.

On the \texttt{fraudecom} dataset (Table \ref{tab:exact_fraudecom}), all CleanLab and micro-model methods again perform comparably, and BaseScore is substantially worse at low FPRs.

Finally, on the \texttt{sparknov} dataset (Table \ref{tab:exact_sparknov}), micro-model methods do slightly better than CleanLab though sometimes this is achieved through an OOT split and sometimes not. The advantage again fades at higher FPR.

\input{tables/known_table_cloud.tex}

\subsection{Unknown Noise Level}

In this set of experiments we always see micro-models perform as well or better than CleanLab, and the choice of using the \textbf{Shuffled} approach is fairly clear. We do not compare the BaseScore method in these experiments as this only works when the noise level is known (we will generally not know what score to use as a cutoff for noise). Again, we show the results for \texttt{cloud} here and other datasets in Appendix \ref{results}.

On the \texttt{cloud} dataset (Table \ref{tab:full_cloud}), micro-models are generally better than their CleanLab counterparts with respect to OOT/non-OOT, and \textbf{Shuffled} is the best method at every FPR.

On the \texttt{ieeecis} dataset (Table \ref{tab:full_ieeecis}), \textbf{Shuffled} is better than competing methods at low FPRs and is as good at high FPRs. Notably, in the best cases here we were able to precisely target the desired FPR.

On the \texttt{ccfraud} dataset (Table \ref{tab:full_ccfraud}), micro-models perform comparably to CleanLab at all FPR ranges, though in this case the OOT splits give better performance vs. the non-OOT splits. Again we don't see any real improvement over the baseline due to the extreme imbalance in this dataset. 

On the \texttt{fraudecom} dataset (Table \ref{tab:full_fraudecom}), micro-models perform comparably to CleanLab at all FPR ranges, the \textbf{Sorted} method is a notable underperformer here, but otherwise other micro-model approaches exhibit similar results.

Lastly, on the \texttt{sparknov} dataset (Table \ref{tab:full_sparknov}), performance is again comparable across many of the methods and \textbf{Shuffled} is generally a good choice.

\input{tables/unknown_table_cloud.tex}

\subsection{Sorted vs. Shuffled}
We conclude by briefly investigating the performance difference between the \textbf{Sorted} and \textbf{Shuffled} methods. To do this, we take the validation data in \texttt{ieeecis} and slice it into as many segments as we have classifiers in our cleaning ensemble. In the \textbf{Sorted} setting, these slices will line up in time with the training slices used for each micro-model; in the \textbf{Shuffled} setting these are just random (but disjoint) subsets. We then look only at the noisy data in each slice and ask what level of accuracy micro-model $i$ attains on slice $j$. We then plot $\abs{i-j}$ against $acc(i,j)$ an observe the results in Figure \ref{fig:accuracy}. In the \textbf{Sorted} setting we see performance is best when $\abs{i-j}$ is small, i.e. when the micro-model was trained on data that is nearby-in-time to the data it is now being asked to evaluate, and that the accuracy decreases as the time-gap increases. On the other hand, for the \textbf{Shuffled} method the accuracy has no meaningful dependence on $\abs{i-j}$ which is to be expected as the assignment of examples to slices is random. Overall this allows the ensemble to have better average performance across models which is obviously valuable when using a voting scheme to identify noise. We observe a similar trend for other datasets, especially \texttt{cloud} and \texttt{sparknov}.

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{figures/ieeecis_noise_30_ensemble_noise_accuracy.png}
\caption{Accuracy on Noisy Data in \texttt{ieeecis}}
\label{fig:accuracy}
\end{figure}

\section{Conclusion and Summary}

Through our experiments we saw that micro-model methods generally perform as well or better than CleanLab on our benchmark datasets, in both the setting where noise is known as well as where it is unknown. In particular, in only a few sub-experiments (\texttt{cloud} with known noise and an FPR target of $0.5\%$, \texttt{ieeecis} with known noise and low FPR targets) did CleanLab perform substantially better, and in many other cases a micro-model approach had significant improvement over CleanLab. The micro-model approach uses relatively few parameters - one must choose the number of classifiers as well as how to split the training and validation data up - but some choices are necessary in most applications (micro-models or not) and we saw that generally the \textbf{Shuffled} approach yielded acceptable results across the entire range of experiments. 

We also found that simply using the base model score to remove examples is never advisable, often going too far with noise removal, and the reason for this is that the error in this method is highly correlated to the way FPR is calculated relative to a score threshold. 


